A Full Adagrad algorithm with O(Nd) operations

A novel approach is given to overcome the computational challenges of the full-matrix Adaptive Gradient algorithm (Full AdaGrad) in stochastic optimization. By developing a recursive method that estimates the inverse of the square root of the covariance of the gradient, alongside a streaming variant for parameter updates, the study offers efficient and practical algorithms for large-scale applications. This innovative strategy significantly reduces the complexity and resource demands typically associated with full-matrix methods, enabling more effective optimization processes. Moreover, the convergence rates of the proposed estimators and their asymptotic efficiency are given. Their effectiveness is demonstrated through numerical studies.

==> title.tex <==
\title{
Online estimation of the inverse of the Hessian for stochastic optimization with application to universal stochastic Newton algorithms}
\author{Antoine Godichon-Baggioni$^{(*)}$,
Wei Lu$^{(**)}$  and Bruno Portier$^{(**)}$\\
       $(*)$ Sorbonne Université, Laboratoire de Probabilités, Statistique et Modélisation  \\ 
       $(**)$ INSA Rouen Normandie, Laboratoire de Mathématiques de l'INSA \\     
         antoine.godichon$\_$baggioni@upmc.fr,  wei.lu@insa-rouen.fr,  bruno.portier@insa-rouen.fr \\
         \date{}
}
\editor{}
